Robust Trajectory-based Density Estimation for Geometric Structure Recovery: Theory and Applications

With the rise of the Internet of Things, strategies for effectively processing big data are essential for discovering meaningul insights. The time series datasets produced by groups of interconnected devices contain valuable underlying patterns. Recent works have extracted patterns from spatio-temporal datasets to aid in road network generation, activity recognition, and others. The speed and accuracy of the underlying geometry reconstruction are important in these applications. Existing methods such as kernel density estimation (KDE) have been used but are often computationally expensive. We propose modifying edge quadtrees to utilize their effective heirarchical structure. Our modification estimates density using a novel trajectory count function which provides mathematical guarantees on the stability of the count by enforcing an invariance to local perturbations. We evaluate our method's effectiveness at extracting the underlying geometry and representative subsample points. For verification, we compare against a KDE variant at extracting the underlying shape of noisy synthetic trajectories travelling alonng the shape. We compare map extraction from GPS traces against current methods. Our method significantly improves runtime while extracting the geometry better or at least comparably. We also compare against maxmin subsampling on an activity recognition data set and find a significant runtime improvement with comparable performance.

==> paper_folders/Sections/Applications/Activity.tex <==
Describe the methodology for processing here

==> paper_folders/Sections/Applications/StreetMap.tex <==
Describe the methodology for streetmap here.

==> paper_folders/Sections/AuthorBios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{trichmo}}]{Turner Richmond}
is a PhD student advised by Dr. Lobaton in the Active Robotic Sensing Lab at North Carolina State University. He received his B.S. degree in Computer Science from University of North Carolina. His work at NCSU consists of contributing work on analysis of wearable sensors as well as species classification of microscopic fossils  using topological properties of the species.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{lokare}}]{Namita Lokare}
is a Senior Biomedical Algorithm Engineer at LVL Technologies, Inc. She is part of a team that focuses on the research and development of data mining and machine learning algorithms that can solve big data problems on wearable platforms. Prior to LVL Technologies, Inc., Dr. Lokare was a part of the Artificial Intelligence and Machine Learning group at SAS. Her research interests include signal processing, time series analysis, and feature engineering. She has worked on developing novel machine learning algorithms to analyze data from wearable sensors at North Carolina State University. Dr. Lokare earned her Master's in Biomedical Engineering from the University of Southern California and a Ph.D. in Electrical Engineering from North Carolina State University.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Qian-Ge}}]{Qian Ge}
received BS and MS degree in Electrical Engineering from University of Electronic Science and Technology of China and a PhD in Electrical Engineering at North Carolina State University.  She is working with Dr. Edgar Lobaton at Active Robotic Sensing (ARoS) Laboratory on computer vision and machine learning. Her research interests are robust image segmentation using deep learning and topological data analysis tools.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ejlobato}}]{Edgar J. Lobaton}
has been an Associate Professor in the Department of Electrical and Computer Engineering at North Carolina State University (NCSU) since 2011. Dr. Lobaton earned his B.S. in Mathematics and Electrical engineering from Seattle University in 2004. He completed his Ph.D. in Electrical Engineering and Computer Sciences from the University of California, Berkeley in 2009. Dr. Lobaton was engaged in research at Alcatel-Lucent Bell Labs in 2005 and 2009. He was awarded the NSF CAREER Award in 2016. He was also awarded the 2009 Computer Innovation Fellows post-doctoral fellowship and conducted research in the Department of Computer Science at the University of North Carolina (UNC) at Chapel Hill from 2009 until 2011. His research focuses on the development of machine learning, estimation theory, and statistical and topological data analysis techniques applied to cyber-physical system in areas such wearable health monitoring, robotics and computer vision.
\end{IEEEbiography}

==> paper_folders/Sections/Datasets/Activity.tex <==
\subsubsection{Activity Recognition Dataset}
\label{sec:ActivityDataset}

In order to evaluate the proposed approach's viability on real time activity recognition, we utilize the NCSU-ADL as presented by Lokare, Zhong, and Lobaton \cite{namitaInventions}.
The dataset contains various physiological and motion data for $10$ individuals as each individual performs a variety of tasks.
From the dataset, the 3-axis accelerometer measurements of the devices on an individual's left wrist and right leg are utilized to classify activity.
Single windows of $1000$ and $2000$ samples are of interest.
Table \ref{tab:ADLDesc} describes the NCSU-ADL dataset where the activity frequency was extracted using autocorrelation.

\begin{table}[]
\centering
\caption{NCSU-ADL Data Description}
\label{tab:ADLDesc}
\begin{tabular}{|l|c|c|c|c|}
\hline
Activity                 & Activity Type                     & \begin{tabular}[c]{@{}l@{}}Activity \\ Frequency\end{tabular}             & \begin{tabular}[c]{@{}l@{}}Sampling \\ Frequency\end{tabular}                     \\ \hline
Rowing                 & Periodic     & 0.40 Hz    & 202 Hz      \\ \hline
Carrying A Box         & Complex      & -          & 202 Hz      \\ \hline
Bicycling              & Periodic     & 1.16 Hz    & 202 Hz      \\ \hline
Resting                & Stationary   & -          & 202 Hz      \\ \hline
Seting Dinner          & Complex      & -          & 202 Hz     \\ \hline
Walking                & Periodic     & 1.42 Hz    & 202 Hz      \\ \hline
Typing                 & Complex      & -          & 202 Hz      \\ \hline
Lying                  & Stationary   & -          & 202 Hz      \\ \hline
\end{tabular}
\end{table}

To classify the activities, the dataset is processed using the method developed by Dirafzoon, Lokare, and Lobaton \cite{alireza_TDE}.
The data stream of the accelerometer data is split up into the windows such that each window contains exactly one activity.
The windows are partitioned in to four subsets such that each contains approximately equal numbers of each activity to allow for four fold cross validation.
The following steps used in \cite{alireza_TDE} are highlighted:
\begin{itemize}
\item Extract four features from the original six raw measurements using PCA for each sample in a window.
\item Perform a time delay embedding on a window.
\item Subsample the embedding utilizing either maxmin subsampling or TRED.
\item Calculate the topologically persistent hole for each feature in a window.
\item Classify the window using a majority vote over the nine nearest neighbors.
\end{itemize}

% \begin{figure*}[h]
% 	\centering
% 	\includegraphics[width=\textwidth]{paper_folders/Images/DataCollection.png} 
% 	\caption{Data collection setup. (a) Individual with wearable sensors, and (b) Physical layout.}
% 	\label{fig:Room}
% \end{figure*}

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\columnwidth]{paper_folders/Images/Panorama_layout.png} 
% 	\caption{\small{Panoramic view of the data collection space highlighting some of the stations.}}
% 	\label{fig:PanoramaRoom}
% \end{figure}

% This section introduces the dataset recorded for this study. As discussed in Section \ref{sec:Introduction}, we aim to predict physiological responses in realistic scenarios. Our dataset focuses on capturing physiological signal and motion information of individuals in scenarios with complex activities and dynamic transitions without the effect of environmental and cognitive / affective factors.

% The data collection was undertaken at North Carolina State University (NCSU) under the Institutional Review Board (IRB) 7799. All participants in the study were healthy individuals in the age group ranging from 18-30 years old. We collected data from 10 volunteers.
% \begin{figure*}[h]
% 	\centering
% 	\includegraphics[width=\textwidth]{paper_folders/Images/Alignment.png} 
% 	\caption{Data alignment and snapshot of protocol, (a) after preprocessing (highlighted orange regions shows a minor misalignment between the peaks caused due to jumps on each device), and (b) after post processing (highlighted green regions showing the corrected alignment via a manual process), and (c) snapshot of the protocol from the TaskTracker App.}
% 	\label{fig:alignment}
% \end{figure*}
% The layout of the space where all the activities were performed is shown in figure \ref{fig:Room} and a panoramic view of the space in figure \ref{fig:PanoramaRoom}. We focus on activities of daily life (ADL), including periodic (e.g. walking, bicycling), non-periodic (e.g. setting up a dinner table), and stochastic (e.g. typing a document). The participants had to undergo a 2-hour session for training, placing sensors, and data collection (approximately 1 hour). The following tasks were included in the protocol:
% \begin{itemize}
% \item{Row on a rowing machine}
% \item{Move a 20 lb object from one table to another}
% \item{Ride an exercise bicycle}
% \item{Rest on a chair for three minutes}
% \item{Set up dinner and clean up the table}
% \item{Walk on the treadmill}
% \item{Drink water}
% \item{Type a one-page document}
% \item{Lie down for three minutes}
% \end{itemize}

% In order to ensure that we capture enough transitions between the different activities, the participants were asked to perform short activities (e.g., moving a 20 lb object) four times throughout the protocol, and longer activities (e.g., walking on the treadmill) two times. Participants were also asked to perform complex activities such as typing a document or setting up a dinner table at their own pace. The first half of the protocol was the same as the second half of the protocol. This was done so we can use the first half for training and the second for prediction in order to mimic more realistic scenarios in which only historic information is available to predict future instances. The sensors used for data collection are:
% \begin{itemize}
% \item{\it{Bioharness}}: This sensor \cite{BioHarness} is an off-the-shelf sensor that can measure subject's heart rate (beats per minute), breathing rate (breaths per minute), acceleration (g), skin temperature ($^\circ$C), and activity levels. This device has an adjustable chest strap and it is worn by the volunteer throughout the data collection process. We collected accelerometer, EKG (electrocardiogram), and breathing rate. The sampling rate was 100 Hz, 250 Hz, and 25 Hz, respectively. %Hailstone el al. \cite{hailstone2011reliability} conducts experiments of 12 subjects on various activities and demonstrates the reliability and validity of measuring respiratory rate with Zephyr BioHarness (a light and flexible wearable chest band) during exercises of varying intensity. One of these devices was worn by the participants.  

% \item{\it{Shimmer Platform}}: Each sensor in this platform \cite{Shimmer} contains an off-the-shelf inertial measurement unit which has a 3-axis low-noise accelerometer, a 3-axis gyroscope and a 3-axis magnetic sensor, which measures acceleration, orientation, and magnetic field respectively.  Five of these devices were worn: two on the wrists, two on the legs, and one on the chest. The sampling rate for these devices was set to 202 Hz. In addition to the IMU unit, the Shimmer sensor \cite{Shimmer} on the chest can record EKG signals. We use this sensor to record the EKG measurements at a sampling rate of 202 Hz.

% \item{\it{Smartphone}}: A Motorolla Moto E (2nd Generation) was used in the experiment to give instructions to the user. The user was given instructions through an application called \textit{TaskTracker} (see figure \ref{fig:alignment} for an snapshot). This tool was developed in house. The user interacts with the protocol by pressing ``Next'', ``Play'', ``Stop'', or ``Previous''. If something goes wrong during an ongoing segment the user can press ``Previous'' to go back to the last segment. The App beeps when the task starts or ends and also includes a countdown timer for certain instructions. This helped us to sync between activities and also allows the participant to move at their own pace and indicate when the activity is complete and are ready to move on to the next task. The interactions with the App are stored locally and used as groundtruth for the activity labels. We also use an application called \textit{ScienceJournal} \cite{ScienceJournal} to record the phone's accelerometer data (x, y, and z axes) for alignment purpose. 
% \end{itemize}



% For this study, we use the respiratory and heart rate measurements from the BioHarness sensor, and accelerometer data from Shimmer sensors. We also use the accelerometer data from the smartphone and BioHarness sensor, but only for data alignment purpose --- this is discussed in Section \ref{sec:DataAlignment}. Prior studies have used smarphone accelerometer data and have shown that even though it is possible to do activity recognition with smartphone data, they are not suitable for activities and motion that incorporate upper limb motion \cite{shoaib2016complex}. Motion artifacts (caused due to movement of the sensor while recording) and poor contact of the sensor can influence the heart rate and respiration rate measurements thus making them unusable in the analysis. According to \cite{kim2013measurement, doi:10.1080/1091367X.2011.615671}, the BioHarness was found to provide reasonably accurate heart rate and respiratory rate  measurements during exercises of varying intensity. In our experiments we noticed consistent good signal quality when the sensor was properly secured to the individual. However, several individuals had low quality signals with motion artifacts when the BioHarness had poor contact with the skin. Due to this issue, only the data from 5 subjects is used for this study.


% %This is for item 1, 3 in More Clarification
% Figure \ref{fig:Dataset} shows a snapshot of the different data streams that are used. The figure also highlights transition regions --- these are the times when a subject was switching between activities. It is worth pointing out that the physiological quantities vary during these transition regions; we can see for instance a clear drop in heart rate and respiration rate in the highlighted green regions in figure \ref{fig:Dataset}. 

==> paper_folders/Sections/Datasets/Biobot.tex <==
\subsection{Biobot Dataset}

\TR{Please review this section Dr. Lobaton to make sure I understood the use of TRED in future CINEMa projects. I guess we can decide if we want to remove this section or not (I think as of now, there's not quite enough data).}

The biobot dataset is concerned with a swarm of $\textit{Gromphadorhina portentosa}$ (Madagascar hissing) cockroaches which are outfitted with a wireless neuro-stimulation backpack system for remote navigation controls.
The swarm explores some space $\mathcal{M} \subset \mathbb{R}^2$.
The dataset is intended to explore how the biobots move in a bounded region, how they behave around boundaries of $\mathcal{M}$, and how they behave in the interior of $\mathcal{M}$.
Insights into the underlying motion behavior of the biobots yields possibilities for exploiting their use in exploring confined or dangerous spaces such as fallen buildings.
We use the dataset to determine how densely the biobots explore a space under no input from their neuro-stimulation backpack.
When undergoing natural motion, the biobots perform two main behaviors.
The first is correlated random walk in which the biobots walk in piecewise linear movements with random changes in direction between the line segments.
The other is wall following in which they walk along the boundary of $\mathcal{M}$ once it has been detected with their antennas.
They switch from wall following back to correlated random walk after some stochastic period of time.
By determining which boundaries have been adequately explored using TRED, the neuro-stimulation backpack can signal to the biobot to exit a well explored boundary and enter correlated random walk to provide more insight into less explored areas of the space.


\TR{Once we know how many roaches we use, the duration of time they explore, and all of the space types they explore, we can add that to the section.  Probably will come after I start running some code on the data to determine how many we need to utilize to get desired results.}



==> paper_folders/Sections/Datasets/DatasetIntroduction.tex <==
\section{Real Data Evaluation}

\subsection{Datasets} \label{Sec:Datasets}

\EL{Based on the fact that we will have a separate section on synthetic, we may want to split the data description and evaluation into two sections: ``Activity Recognition Evaluation'' and ``Streetmap Reconstruction Evaluation.''}

In the following section, we aim to provide insight into datasets which are well suited to benefit from the presented approach.
While the datasets vary in application type widely, each is able to be embedded into a spatio-temporal space.
The objective when working with each of the datasets is remove outlying samples resulting from noise while extracting the underlying topological structure of the dataset.


\input{paper_folders/Sections/Datasets/Activity}

\input{paper_folders/Sections/Datasets/StreetMap}

% \input{paper_folders/Sections/Datasets/Biobot}

==> paper_folders/Sections/Datasets/StreetMap.tex <==
\subsection{Streetmap Dataset}
\label{sec:SMDataset}
Ahmed, Karagiorgou, Pfoser, and Wenk \cite{WenkMap} provide a collection of a diverse set of tracking datasets and algorithms.
The datasets provided contain both the tracking dataset as well as the ground truth with associated evaluation metrics for evaluation.
The road networks included vary in covered area from $15.6 km^{2}$ to $168 km^{2}$.
We provide an overview of the data collection characteristics for each of the maps and the corresponding characteristics of the ground truth data structures from OpenStreetMap in Table \ref{table:mapTrackingTable}.
We note the methods of data collection vary slightly among the datasets with Athens large and small being collected from the routes of school buses, Berlin collected from a taxi fleet, and Chicago collected from university shuttle buses.

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|}
\cline{2-9}
 & \multicolumn{4}{c|}{Collection Characteristics} & \multicolumn{4}{c|}{Ground Truth Characteristics} \\ \cline{2-9} 
 & Trajectories & \begin{tabular}[c]{@{}c@{}}Sampling\\ rate (s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Trajectory\\ Length (km)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Speed\\ (km/h)\end{tabular} & Vertices & Edges & \begin{tabular}[c]{@{}c@{}}Length\\ (km)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Area\\ (km)\end{tabular} \\ \hline
\multicolumn{1}{|c|}{Athens Large} & 120 & 30.14 & 6,781 & 20.16 & 32,212 & 39,699 & 2,000 & 12 x 14 \\ \hline
\multicolumn{1}{|c|}{Athens Small} & 129 & 34.07 & 433 & 19.55 & 2,694 & 3,436 & 193 & 2.6 x 6 \\ \hline
\multicolumn{1}{|c|}{Berlin} & 26,831 & 41.98 & 41,116 & 35.23 & 5,894 & 6,839 & 360 & 6 x 6 \\ \hline
\multicolumn{1}{|c|}{Chicago} & 889 & 3.61 & 2,869 & 33.14 & 9,429 & 11,801 & 61 & 7 x 4.5 \\ \hline
\end{tabular}%
}
\caption{Overview of mapping dataset characteristics}
\label{table:mapTrackingTable}
\end{table*}

==> paper_folders/Sections/Results/ResultsIntroduction.tex <==
\subsection{Evaluation}

Below we present the results of applying TRED on the datasets presented in section \ref{Sec:Datasets}.  

\input{paper_folders/Sections/Results/Activity}
\input{paper_folders/Sections/Results/StreetMap}
